Intrinsic alignments of BOSS LOWZ galaxies II: Impact of shape measurement methods

Measurements of intrinsic alignments of galaxy shapes with the large-scale density field, and the inferred intrinsic alignments model parameters, are sensitive to the shape measurement methods used. In this paper we measure the intrinsic alignments of the Sloan Digital Sky Survey-III (SDSS-III) Baryon Oscillation Spectroscopic Survey (BOSS) LOWZ galaxies using three different shape measurement methods (re-Gaussianization, isophotal, and de Vaucouleurs), identifying a variation in the inferred intrinsic alignments amplitude at the 40% level between these methods, independent of the galaxy luminosity or other properties. We also carry out a suite of systematics tests on the shapes and their two-point correlation functions, identifying a pronounced contribution from additive PSF systematics in the de Vaucouleurs shapes. Since different methods measure galaxy shapes at different effective radii, the trends we identify in the intrinsic alignments amplitude are consistent with the interpretation that the outer regions of galaxy shapes are more responsive to tidal fields, resulting in isophote twisting and stronger alignments for isophotal shapes. We observe environment dependence of ellipticity, with brightest galaxies in groups being rounder on average compared to satellite and field galaxies. We also study the anisotropy in intrinsic alignments measurements introduced by projected shapes, finding effects consistent with predictions of the nonlinear alignment model and hydrodynamic simulations. The large variations seen using the different shape measurement methods have important implications for intrinsic alignments forecasting and mitigation with future surveys.

==> referee_report <==
> Assistant Editor's Comments:
> Editor
> Comments to the Author:
> As you have not chosen to pay for colour printing, please ensure
> that your figures are legible when printed in black & white, or
> provide separate sets of figures for the print and online editions
> of the journal.

We have slightly modified Figure 2 and 12 for better legibility in
black & white. We prefer to keep other figures as they are.

> Reviewer's Comments:
> Reviewer: 1

> Comments to the Author
> This paper presents a study of the intrinsic (i.e., non-lensing)
> alignment of galaxy ellipticity vectors, one of the most important
> systematics affecting weak lensing measurements. It focuses on the 
> effect of different shape measurement techniques on IA statistics.

> Overall the paper is well-written, and the analysis quite 
> straightforward -- so I am happy to recommend the paper for 
> publication. However I have a few suggestions the authors may wish 
> to consider.

We thank the referee for the positive report and the helpful
suggestions.  Our edits in the paper are shown in blue.

> Several figure captions refer to a function (eg xi_g+) without 
> description or reference to the text. It might improve readibility to
> describe these plotted quantities briefly in words in the captions.

We have added a few clarifying words along with references to the
relevant equations in the captions.

> In S3.3 the different shape measurements studied in the paper are
> presented. But why these and not the many others on the market? Do
> these methods span the behaviour that may be expected from all
> methods (see eg the GREAT3 paper by Mandelbaum++)? Some discussion
> of this point would be very useful, and help place the results of
> the paper in the context of ongoing and future surveys.

We are using the shape measurements that are readily available and
have been used in several papers studying intrinsic alignments in SDSS
galaxies. The primary focus of our paper is to resolve some of the
discrepancies in older SDSS IA analyses done using different shape
measurements and methodology. We agree with the referee that doing
similar comparisons with other shape measurements would be useful, but
this will require redoing the SDSS imaging analysis.  The SDSS imaging
pipeline is notoriously difficult to run and modify, so a re-analysis
using other shape measurement methods would take an amount of
resources that is well outside the scope of what makes sense for this
work.  We have added a brief statement in section 3.3 highlighting the
reasons for our choices of shape measurement methods, and also how we
might make some (admittedly limited) inferences that could apply to
other methods.

> Fig.1 caption: panel (b) is not as a function of redshift but of
> Rcirc. Also in this caption the remark about the 'likely' cause of
> the spikes in the deVaucouleurs ellipticities should be
> confirmed. Either it is or not caused by discretization of model
> parameters - the authors should investigate this point and not speculate.

We have corrected the error in the caption for panel (b).

To clarify the comments about discretization of model parameters:
certain parameters including ellipticity are definitely discretized
during the fit, and when we look at 2d contour plots of ellipticity
vs. other parameters that are discretized (e.g., position angle) we
also see such features at regular intervals.  There are also comments
about this in the Stoughton et al 2002 paper to which we originally
referred in the text, and on the SDSS DR12 data release website,
implying that the issue has not changed in the many subsequent data
releases since 2002.

However, we agree that an issue of this sort is too complex to discuss
in a figure caption and that we should not have used the word "likely"
which implies some uncertainty in this explanation.  We have changed
those comments to a statement that the reader should see the text for
discussion of the spiky features.  Unlike the caption, the text as
originally written did not have this confusing ambiguity in it.
 
> S4.4 discusses possible explanations for the causes of IA amplitude 
> found with the different methods. The point of multiplicative bias
> is mentioned here, but in my view dismissed too
> simplistically. Differences in e_rms do not only reflect differences
> in noise level, but can also point to real ellipticity gradients. A
> combination of different noise levels and ellipticity gradients can
> produce multiplicative biases that either boost or suppress the IA
> signal in any method.

We agree with the referee that ellipticity gradients can also lead to
different IA amplitude. However, ellipticity gradients alone cannot
explain the gradients in alignment angle \theta as shown in figure 9;
those require some kind of isophotal twisting as we pointed out in
section 4.4.  Also, we have shown in the sec 4.1 that isophotal shapes
have lower RMS ellipticity, which suggests that if galaxies have the
same alignment with the tidal field but an ellipticity gradient, the
IA amplitude should be lower for isophotal shapes, not higher. We have
expanded the discussion in sec. 4.4, highlighting these and other
relevant points.

Finally, we note that the original version of the paper did acknowledge that we cannot rule out
multiplicative bias playing a role in some aspects of the results, so we think that we have been
appropriately cautious about this already.

> S5, conclusions: the first paragraph speculates about the
> differences found being due to different methods effectively
> measuring shapes at different radii. It strikes me that if this is
> indeed the effect, then a more direct and controlled way to study it
> is to use the same method with different parameters (eg measure e at
> different isophotal levels, use a different weight radius in the
> moments, etc). Perhaps the authors can add some comments to this effect.

We agree with the referee that it will be very useful to test shape
gradients in a controlled way. As stated earlier, it is non-trivial to
do using SDSS data. We have added a line in the discussion, suggesting
that future studies carry out such tests.  However, we hope that our
modifications of section 4.4 have helped further convince the referee
that our proposed explanation is plausible.

